Retrieval with Learned Similarities

Retrieval plays a fundamental role in recommendation systems, search, and natural language processing (NLP) by efficiently finding relevant items from a large corpus given a query. Dot products have been widely used as the similarity function in such tasks, enabled by Maximum Inner Product Search (MIPS) algorithms for efficient retrieval. However, state-of-the-art retrieval algorithms have migrated to learned similarities. These advanced approaches encompass multiple query embeddings, complex neural networks, direct item ID decoding via beam search, and hybrid solutions. Unfortunately, we lack efficient solutions for retrieval in these state-of-the-art setups. Our work addresses this gap by investigating efficient retrieval techniques with expressive learned similarity functions. We establish Mixture-of-Logits (MoL) as a universal approximator of similarity functions, demonstrate that MoL's expressiveness can be realized empirically to achieve superior performance on diverse retrieval scenarios, and propose techniques to retrieve the approximate top-k results using MoL with tight error bounds. Through extensive experimentation, we show that MoL, enhanced by our proposed mutual information-based load balancing loss, sets new state-of-the-art results across heterogeneous scenarios, including sequential retrieval models in recommendation systems and finetuning language models for question answering; and our approximate top-$k$ algorithms outperform baselines by up to 66x in latency while achieving >.99 recall rate compared to exact algorithms.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> figure_learned_similarity.tex <==
\begin{figure*}[t]
    \caption{\todo{Examples of learned simlairity scores}}
    \label{fig:learned_similarity}
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{figure/placeholder_5x8.png}
        \caption{Tree traversal similarity}
        \label{fig:leared_similarity:tree}
    \end{subfigure}%
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{figure/placeholder_5x8.png}
        \caption{Path traversal similarity}
        \label{fig:leared_similarity:path}
    \end{subfigure}%
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{figure/placeholder_5x8.png}
        \caption{Mixture of logits similarity}
        \label{fig:leared_similarity:mol}
    \end{subfigure}%
\end{figure*}

==> figure_topk_algorithm.tex <==
\begin{figure*}[t]
    \caption{\todo{Illustration of top $K$ algorithms}}
    \label{fig:algorithm:topk}
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{figure/placeholder_5x8.png}
        \caption{Brute force}
        \label{fig:algorithm:bruteforce}
    \end{subfigure}%
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{figure/placeholder_5x8.png}
        \caption{Exact two pass algorithm}
        \label{fig:algorithm:twopass}
    \end{subfigure}%
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{figure/placeholder_5x8.png}
        \caption{Union of top $K$ of each embedding set}
        \label{fig:algorithm:topkunion}
    \end{subfigure}%
    \\
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{figure/placeholder_5x8.png}
        \caption{Top $K$ by average dot product score}
        \label{fig:algorithm:topkavg}
    \end{subfigure}%
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{figure/placeholder_5x8.png}
        \caption{Top $k$ by max dot product score}
        \label{fig:algorithm:topkmax}
    \end{subfigure}%
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.95\linewidth]{figure/placeholder_5x8.png}
        \caption{Combined top $K$}
        \label{fig:algorithm:topkcomb}
    \end{subfigure}%
\end{figure*}

==> results_recsys.tex <==
amzn-books (11-16c ep180):

================amzn-books===============
algorithm,HR@1,HR@5,HR@10,HR@50,HR@100,BatchTimeMsAvg,BatchTimeMsDev
MoLBruteForceTopK,0.017822265625,0.0467529296875,0.0667724609375,0.136962890625,0.177490234375,128.359,0.300
MoLNaiveTopK5,0.0181884765625,0.0430908203125,0.060302734375,0.0830078125,0.0843505859375,20.474,0.066
MoLNaiveFaissTopK5,0.015869140625,0.03662109375,0.05126953125,0.0682373046875,0.0693359375,16.937,0.233
MoLNaiveTopK10,0.0179443359375,0.0457763671875,0.065673828125,0.10498046875,0.1124267578125,20.624,0.121
MoLNaiveTopK50,0.017822265625,0.046875,0.0667724609375,0.134765625,0.1649169921875,21.596,0.079
MoLNaiveTopK100,0.017822265625,0.046630859375,0.0670166015625,0.13525390625,0.1712646484375,23.320,0.079
MoLAvgTopK200,0.0172119140625,0.0428466796875,0.0604248046875,0.104248046875,0.1181640625,1.129,0.035
MoLAvgTopK500,0.0172119140625,0.045654296875,0.064453125,0.1175537109375,0.144287109375,1.172,0.042
MoLAvgTopK1000,0.017578125,0.0460205078125,0.06640625,0.125732421875,0.1556396484375,1.121,0.045
MoLAvgTopK2000,0.017822265625,0.04638671875,0.0665283203125,0.1298828125,0.1634521484375,1.198,0.023
MoLAvgTopK4000,0.0179443359375,0.0467529296875,0.0667724609375,0.1309814453125,0.168212890625,2.051,0.014
MoLCombTopK5_200,0.0181884765625,0.046142578125,0.0660400390625,0.1171875,0.134765625,20.749,0.067
MoLCombTopK50_500,0.017822265625,0.0469970703125,0.067138671875,0.1358642578125,0.16943359375,22.121,0.072
MoLCombTopK100_1000,0.017822265625,0.046630859375,0.0670166015625,0.1357421875,0.174560546875,24.018,0.126
MoLNaiveTopK200,0.017822265625,0.046630859375,0.06689453125,0.13671875,0.1766357421875,26.545,0.116
MoLAvgTopK8000,0.0179443359375,0.0467529296875,0.0670166015625,0.1334228515625,0.17138671875,3.790,0.010
MoLCombTopK200_2000,0.017822265625,0.0467529296875,0.06689453125,0.13720703125,0.1767578125,28.013,0.114

================amzn-books===============
algorithm,HR@1,HR@5,HR@10,HR@50,HR@100,BatchTimeMsAvg,BatchTimeMsDev
MoLBruteForceTopK,1.0,1.0,1.0,1.0,1.0,129.615,1.444
MoLNaiveTopK5,0.784423828125,0.784423828125,0.784423828125,0.784423828125,0.784423828125,20.919,0.995
MoLNaiveFaissTopK5,0.6297607421875,0.6297607421875,0.6297607421875,0.6297607421875,0.6297607421875,16.975,0.233
MoLNaiveTopK10,0.872314453125,0.872314453125,0.872314453125,0.872314453125,0.872314453125,20.956,0.618
MoLNaiveTopK50,0.96728515625,0.96728515625,0.96728515625,0.96728515625,0.96728515625,23.623,2.388
MoLNaiveTopK100,0.9847412109375,0.9847412109375,0.9847412109375,0.9847412109375,0.9847412109375,26.320,2.788
MoLAvgTopK200,0.7545166015625,0.7545166015625,0.7545166015625,0.7545166015625,0.7545166015625,1.126,0.043
MoLAvgTopK500,0.846923828125,0.846923828125,0.846923828125,0.846923828125,0.846923828125,1.102,0.005
MoLAvgTopK1000,0.8975830078125,0.8975830078125,0.8975830078125,0.8975830078125,0.8975830078125,1.110,0.031
MoLAvgTopK2000,0.9329833984375,0.9329833984375,0.9329833984375,0.9329833984375,0.9329833984375,1.312,0.163
MoLAvgTopK4000,0.956787109375,0.956787109375,0.956787109375,0.956787109375,0.956787109375,2.212,0.195
MoLCombTopK5_200,0.919921875,0.919921875,0.919921875,0.919921875,0.919921875,23.075,2.203
MoLCombTopK50_500,0.984130859375,0.984130859375,0.984130859375,0.984130859375,0.984130859375,24.923,2.612
MoLCombTopK100_1000,0.9927978515625,0.9927978515625,0.9927978515625,0.9927978515625,0.9927978515625,26.889,2.700

================ml-20m===============
algorithm,HR@1,HR@5,HR@10,HR@50,HR@100,BatchTimeMsAvg,BatchTimeMsDev
MoLBruteForceTopK,0.1013769656419754,0.267089307308197,0.3674265146255493,0.6245586276054382,0.7246214747428894,2.732,0.010
MoLNaiveTopK5,0.07006130367517471,0.17901988327503204,0.22985276579856873,0.2884838879108429,0.2890254259109497,1.612,0.050
MoLNaiveFaissTopK5,0.07134656608104706,0.16565458476543427,0.21055938303470612,0.2697248160839081,0.27109673619270325,5.720,0.090
MoLNaiveTopK10,0.09604095667600632,0.23428620398044586,0.30218854546546936,0.40383267402648926,0.41151538491249084,1.647,0.055
MoLNaiveTopK50,0.1022217720746994,0.26721206307411194,0.36483433842658997,0.5914667248725891,0.6637663841247559,1.638,0.053
MoLNaiveTopK100,0.10227231681346893,0.2687644958496094,0.36882007122039795,0.6170637011528015,0.7065627574920654,2.312,0.021
MoLAvgTopK200,0.10116034746170044,0.26641058921813965,0.36674776673316956,0.6155906915664673,0.6990822553634644,1.190,0.043
MoLAvgTopK500,0.10116756707429886,0.2668510377407074,0.36720266938209534,0.6238510012626648,0.7219570875167847,1.222,0.048
MoLAvgTopK1000,0.10132642090320587,0.2670748829841614,0.3674120604991913,0.6244575381278992,0.7242171168327332,1.224,0.051
MoLAvgTopK2000,0.10134807974100113,0.267089307308197,0.36744093894958496,0.6246163845062256,0.7245709300041199,1.340,0.037
MoLCombTopK5_200,0.10228675603866577,0.2688439190387726,0.36951327323913574,0.6179879307746887,0.7010679244995117,1.856,0.058
MoLCombTopK50_500,0.10229397565126419,0.26905331015586853,0.3697226643562317,0.6254828572273254,0.7235311269760132,2.040,0.037

================ml-20m===============
algorithm,HR@1,HR@5,HR@10,HR@50,HR@100,BatchTimeMsAvg,BatchTimeMsDev
MoLBruteForceTopK,0.9868946671485901,0.9974439144134521,0.9994945526123047,1.0,1.0,2.775,0.023
MoLNaiveTopK5,0.5769244432449341,0.687789261341095,0.692785918712616,0.6930386424064636,0.6930386424064636,1.608,0.060
MoLNaiveFaissTopK5,0.5573927760124207,0.6290065050125122,0.6328189969062805,0.633006751537323,0.633006751537323,5.690,0.114
MoLNaiveTopK10,0.832605242729187,0.83274245262146,0.8328218460083008,0.8328579664230347,0.8328579664230347,1.618,0.053
MoLNaiveTopK50,0.985724925994873,0.9857321381568909,0.9857321381568909,0.9857321381568909,0.9857321381568909,1.676,0.094
MoLNaiveTopK100,0.9970973134040833,0.9971045255661011,0.9971045255661011,0.9971045255661011,0.9971045255661011,2.374,0.064
MoLAvgTopK200,0.9720491170883179,0.9874217510223389,0.9897900819778442,0.9902521967887878,0.9902521967887878,1.209,0.046
MoLAvgTopK500,0.9817246794700623,0.9937325119972229,0.9958409667015076,0.9963680505752563,0.9963680505752563,1.213,0.050
MoLAvgTopK1000,0.9847501516342163,0.9956098794937134,0.9977038502693176,0.9982237219810486,0.9982237219810486,1.206,0.044
MoLAvgTopK2000,0.9862953424453735,0.9968951344490051,0.9989674687385559,0.9994873404502869,0.9994873404502869,1.332,0.038
MoLCombTopK5_200,0.9935736656188965,0.9935881495475769,0.9936025738716125,0.9936025738716125,0.9936025738716125,1.887,0.082
MoLCombTopK50_500,0.9993212819099426,0.9993284940719604,0.9993284940719604,0.9993284940719604,0.9993284940719604,2.088,0.088

==> sec_overview.tex <==
\section{Overview}
\label{sec:overview}

\subsection{MoL learned similarity function}
\label{sec:overview:mol}

\todo{JZ: Add a description of the model architecture in Figure~\ref{fig:mol}}

\input{figure_mol}

\todo{JZ: Add a figure to show the details of how to compute learned similarity in~\cite{zhai23kdd}. It shows how to go from $n$ embeddings of items and $n$ embeddings of query to $n\times n$ embeddings in the set. And then how the $n\times n$ embeddings are weighted with MoL into the learned similarity score.}

Table~\ref{table:notations} summarizes the notations in this paper.

\input{table_notations}

\subsection{Problem specification}

General problem setup
\begin{itemize}
    \item Input: Given a feature vector $q$, an integer $k$, and a similarity function $f(q, x) \to \mathbb{R}$, from a set of items $\mathbb{X}$, return the top $K$ items $x \in \mathbb{X}$ with the highest utility according to $f$.
    \item The feature vector can be either the original feature vector or post processed feature vector. For the concern of this work, they are inter-exchangeable and are all referred to as feature vector.
    \item The utility function $f$ is computed using the feature vector of the query and the feature vector of the item. 
    \item The feature vector of the item is given and static for all queries.
    \item The feature vector of the query is dynamic and unknown upfront.
    \item In MoL, the feature vector of the item is mapped to a set of embeddings via a learned model. In theory, the set of embeddings can change even with the same item because the model's behavior at inference can be non-deterministic. For the concern of this work, we assume each feature vector of an item is mapped to a set of embeddings (or a feature vector) that are static.
    \item In MoL, the feature vector of the query is also mapped to a list of embeddings via a learned model. These embeddings are computed on-the-fly at the inference time because the query is dynamic and unknown upfront.
    \item MoL needs the feature vectors or the embeddings of the query and item to compute the learned similarity score.
\end{itemize}

Specific problem setup for the MoL and embeddings in~\citep{zhai23kdd}
\begin{itemize}
    \item The set of $P$ embeddings is constructed by $P_q$ embeddings of the query and $P_x$ embeddings of the items, where $P=P_q\times P_x$, i.e., cross products of the embeddings for the query and the item. For example, if there are $4$ embeddings of the query and $2$ embeddings of the items, then the total number of embedding sets will be $4\times 2=8$.
\end{itemize}



==> table_ml_model_efficiency.tex <==

\begin{table*}[h]
\small
\begin{center}
  \begin{tabular}{clllllll}
    \toprule
                       & \bf Method     & \bf HR@10              & \bf HR@50        & \bf MRR            & \rebuttalrevision{Time/Epoch} \\
    \midrule
\multirow{4}{*}{\mlonem} & SASRec       & .2818               & .5470               & .1352              & \rebuttalrevision{37s} \\
                         & SASRec + MoL & .3034 (+7.7\%)      & .5655 (+3.4\%)      & .1448 (+7.1\%)     & \rebuttalrevision{44s (+18.9\%)} \\
                         & HSTU         & .3332               & .5956               & .1579              &  \rebuttalrevision{41s}\\
                         & HSTU + MoL   & \bf .3460 (+3.8\%)  & \bf .6048 (+1.5\%)  & \bf .1673 (+6.0\%) & \rebuttalrevision{46s (+12.2\%)} \\
    \midrule
\multirow{4}{*}{\mltwentym} & SASRec       & .2883              & .5484               & .1375               & \rebuttalrevision{197s} \\
                            & SASRec + MoL & .3124 (+8.4\%)     & .5685 (+3.7\%)      & .1551 (+12.8\%)     & \rebuttalrevision{449s (+127.9\%)} \\
                            & HSTU         & .3557              & .6146               & .1800               & \rebuttalrevision{526s} \\
                            & HSTU + MoL   & \bf .3697 (+3.9\%) & \bf .6244 (+1.6\%)  & \bf .1880 (+4.4\%)  & \rebuttalrevision{773s (+47.0\%)} \\
    \midrule
\multirow{4}{*}{\amzn} & SASRec           & .0306               & .0754               & .0153               & \rebuttalrevision{506s} \\ % 306s -> 506 (bs reduction) \\
                       & SASRec + MoL     & .0402 (+31.4\%)     & .0970 (+28.6\%)     & .0203 (+32.7\%)     & \rebuttalrevision{964s (+90.5\%)} \\
                       & HSTU             & .0469               & .1066               & .0233               & \rebuttalrevision{1883s} \\ % 2002 -> 1883 \\
                       & HSTU + MoL       & \bf .0613 (+30.7\%) & \bf .1292 (+21.2\%) & \bf .0315 (+35.2\%) & \rebuttalrevision{2236s (+18.7\%)} \\ % 2415 -> 2236
  \bottomrule
\end{tabular}
%\vspace{-0.5em}
\caption{Evaluation of recommendation retrieval performance, utilizing the next-item prediction task. \rebuttalrevision{Note that these results are identical to those reported in Table~\ref{tbl:public-data-full-appendix} but with relative gains (MoL vs dot product) and training cost changes illustrated under different sequential encoder backbones.}} % with different similarity functions and under different backbones.}
\label{tbl:ml-model-efficiency}
\end{center}
\vspace{-1em}
\end{table*}


==> table_ml_regularization_nlp_ablation.tex <==

% https://proceedings.neurips.cc/paper_files/paper/2023/hash/91228b942a4528cdae031c1b68b127e8-Abstract-Conference.html
% https://github.com/Lunarmony/vectordb_vldb24/blob/main/nanoDPR/METRICS-final-l512-ln.md
\begin{table}
\small
\begin{center}
  \begin{tabular}{llllll}
    \toprule
    \bf Method  & \bf HR@1 & \bf HR@10         & \bf HR@100      & \bf MRR    \\
    \midrule                              
    \multicolumn{5}{l}{\textit{Learned similarities}} \\
     MoL       & \bf 68.4      &  \bf 92.0     & \bf 97.0  & \bf 77.3 \\
     abl. $\mathcal{L}_{MI}$ & 67.3 (-1.6\%) & 91.9 (-0.1\%) & 96.8 (-0.2\%) & 76.7 (-0.8\%) \\
                                    % 67.3 91.9 97.8
  \bottomrule
\end{tabular}
\vspace{0.3em}
\caption{\nlprevision{Ablation studies of $\mathcal{L}_{MI}$ on NQ320K.}}
\label{tbl:model-quality-nlp-ablation}
\vspace{-1em}
\end{center}
\end{table}


==> table_ml_regularization_reco_ablation.tex <==

\begin{table*}
\small
%\vspace{-.5em}
\begin{center}
  \begin{tabular}{cllllll}
    \toprule
                        & \bf Method  & \bf HR@1 & \bf HR@10         & \bf HR@50        &  \bf HR@200    & \bf MRR    \\
    \midrule
% 10/07 @10
% ML-1M (HSTU) [latest]
%                                 | hr@1           hr@10          hr@50          hr@200         ndcg@10        ndcg@50        ndcg@200       mrr           
%HSTU-large +MoL RAIL uid l2 0.1 + mi (**) | 0.0884         0.3465         0.6022         0.7935         0.2010         0.2576         0.2867         0.1712        
%HSTU-large +MoL RAIL uid l2 0.1 - mi ablation | 0.0847 (-4.2%) 0.3417 (-1.4%) 0.6011 (-0.2%) 0.7942 (0.1%) 0.1957 (-2.6%) 0.2532 (-1.7%) 0.2827 (-1.4%) 0.1662 (-2.9%)
%          SASRec uid l2 0.1 + mi | 0.0697 (-21.2%) 0.3036 (-12.4%) 0.5617 (-6.7%) 0.7667 (-3.4%) 0.1696 (-15.6%) 0.2270 (-11.8%) 0.2582 (-9.9%) 0.1441 (-15.8%)
%ML-20M (HSTU)
%                                 | hr@1           hr@10          hr@50          hr@200         ndcg@10        ndcg@50        ndcg@200       mrr           
%HSTU-large +MoL RAIL uid l2 0.1 + mi (**) | 0.1010         0.3698         0.6260         0.8132         0.2195         0.2763         0.3048         0.1881        
%HSTU-large +MoL RAIL uid l2 0.1 - mi ablation  | 0.0994 (-1.5%) 0.3670 (-0.7%) 0.6241 (-0.3%) 0.8128 (-0.0%) 0.2176 (-0.9%) 0.2747 (-0.6%) 0.3034 (-0.4%) 0.1866 (-0.8%)  
%
%Amazon Books
%                                 | hr@1           hr@10          hr@50          hr@200         ndcg@10        ndcg@50        ndcg@200       mrr           
%         HSTU-large +MoL RAIL mi | 0.0156         0.0693         0.1362         0.2144         0.0380         0.0525         0.0642         0.0329        
%HSTU-large +MoL RAIL mi ablation | 0.0139 (-10.9%) 0.0661 (-4.6%) 0.1315 (-3.5%) 0.2153 (0.5%) 0.0368 (-2.9%) 0.0511 (-2.5%) 0.0637 (-0.8%) 0.0323 (-1.5%)
%             SASRec +MoL RAIL mi | 0.0095 (-39.1%) 0.0429 (-38.1%) 0.0915 (-32.8%) 0.1635 (-23.7%) 0.0237 (-37.5%) 0.0341 (-34.9%) 0.0449 (-30.1%) 0.0212 (-35.4%)
\multirow{2}{*}{\mlonem} & MoL   & \bf .0884 & \bf .3465     & \bf .6022    & .7935 & \bf .1712  \\
                         & abl. $\mathcal{L}_{MI}$  & .0847 (-4.2\%) & .3417 (-1.4\%) & .6011 (-0.2\%) & \bf .7942 (0.1\%) & .1662 (-2.9\%) \\
    \midrule
\multirow{2}{*}{\mltwentym} & MoL           & \bf .1010 & \bf .3698 & \bf .6260  & \bf .8132      & \bf .1881   \\
                            & abl. $\mathcal{L}_{MI}$  & .0994 (-1.5\%) & .3670 (-0.7\%) & .6241 (-0.3\%) & .8128 (-0.0\%) & .1866 (-0.8\%) \\
    \midrule
\multirow{2}{*}{\amzn} & MoL                             & \bf .0156  & \bf .0693  & \bf .1362  & .2144 & \bf .0329 \\
                       & abl. $\mathcal{L}_{MI}$         & 0.0139 (-10.9\%) & .0661 (-4.6\%) & .1315 (-3.5\%) & \bf .2153 (0.5\%) & .0323 (-1.5\%) \\
  \bottomrule
\end{tabular}
\vspace{0.3em}
\caption{\nlprevision{Ablation studies of $\mathcal{L}_{MI}$ on MovieLens (\mlonem, \mltwentym) and Amazon Reviews (\amzn).}}
\label{tbl:model-quality-reco-ablation}
\vspace{-1em}
\end{center}
\end{table*}


==> table_topk_v2.tex <==
\begin{table*}[ht]
\small
%\vspace{-0.8em}
\begin{center}
  \begin{tabular}{clllllll}
    \toprule

                        & \bf Method  & \bf HR@1 & \bf HR@5 & \bf HR@10 & \bf HR@50 & \bf HR@100 &  \bf Latency / ms \\                        
    \midrule
\multirow{10}{*}{\mlonem} & \topkbf & 1.00  &	1.00  &	1.00  &	1.00  &	1.00  &	.64$\pm$.03 \\
                       & \topknaive{5}  & .838	& .768	& .681	& .499	& .437	& .95$\pm$.03 \\
                       & \topknaive{10}   & .932	& .905	& .842	& .678	& .618	& .94$\pm$.05\\
                       & \topknaive{50}   & \bf 1.00	& \bf .997	& \bf .999	& .977	& .954	& .95$\pm$.05\\
                       & \topknaive{100}   & \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .995	& \bf .990	& 1.24$\pm$.04\\
                       & \topkavg{200}   &  .980	& .970	& .967	& .958	& .948	& .74$\pm$.06\\
                       & \topkavg{500}   & \bf .992	& \bf .986	& \bf .989	& \bf .990	& \bf .990	& .71$\pm$.04\\
                       & \topkavg{1000}   &  \bf .996	& \bf .994	& \bf .998	& \bf .997	& \bf .999	& .72$\pm$.03\\
                       %& \topkavg{2500}   &  \bf .996	& \bf .995	& \bf .999	& \bf 1.00	& \bf 1.00	& .86$\pm$.03\\
                       & \topkcomb{5}{200}  & \bf 1.00	& \bf .997	& \bf .988	& .975	& .960	& 1.09$\pm$.08 \\
                       & \topkcomb{50}{500}   & \bf 1.00	& \bf .999	& \bf .999	& \bf .998	& \bf .997	& 1.13$\pm$.04  \\
    \midrule
\multirow{10}{*}{\mltwentym} & \topkbf & 1.00	& 1.00	& 1.00	& 1.00	& 1.00	& 3.08$\pm$.02\\
                       & \topknaive{5}  & .755	& .702	& .645	& .467	& .402	& 1.19$\pm$.05\\
                       & \topknaive{10}   & .946	& .876	& .817	& .645	& .564	& 1.17$\pm$.05\\
                       & \topknaive{50}   & \bf .993	& \bf .986	& .977	& .931	& .900	& 1.55$\pm$.03\\
                       & \topknaive{100}   &	\bf .998	& \bf .997	& \bf .994	& .979	& .966	& 2.26$\pm$.03 \\
                       & \topkavg{200}   &	\bf .992	& \bf .992	& \bf .992	& .980	& .958	& .76$\pm$.04\\
                       & \topkavg{500}   &	\bf .992	& \bf .993	& \bf .995	& \bf .995	& \bf .993	& .77$\pm$.04\\
                       & \topkavg{1000}    & \bf .992	& \bf .994	& \bf .996	& \bf .998	& \bf .997	& .75$\pm$.03\\
                       %& \topkavg{2500}       & \bf .993	& \bf .994	& \bf .996	& \bf .998	& \bf .999	& 1.29$\pm$.03	\\%&	\bf 1.00	&	\bf 1.00 &	\bf 	.999	&	\bf .997 &	\bf 	.995 & \bf	7.27$\pm$.05\\
                       & \topkcomb{5}{200}    & \bf 1.00	& \bf .998	& \bf .998	& .983	& .962	& 1.32$\pm$.06\\
                       & \topkcomb{50}{500}   & \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .999	& \bf .996	& 1.85$\pm$.03\\
    \midrule
\multirow{13}{*}{\amzn} & \topkbf & 1.00	& 1.00	& 1.00	& 1.00	& 1.00	& 149.02$\pm$.49\\
                       & \topknaive{5}  & .907	& .915	& .809	& .509	& .396	& 20.17$\pm$.06\\
                       & \topknaive{10}    & .936	& \bf .986	& .914	& .698	& .561	& 20.33$\pm$.06\\
                       & \topknaive{50}    & \bf .993	& \bf .992	& \bf .994	& .956	& .902	& 21.09$\pm$.04\\
                       & \topknaive{100}  & \bf 1.00	& \bf .995	& \bf .996	& \bf .985	& .959	& 22.53$\pm$.06\\
                       & \topkavg{200}   	& \bf 1.00	& .978	& .948	& .845	& .767	& .68$\pm$.03\\
                       & \topkavg{500}   	& \bf 1.00	& \bf .992	& \bf .996	& .919	& .875	& .68$\pm$.03\\
                       & \topkavg{1000}   	& \bf 1.00	& \bf 1.00	& \bf .996	& .963	& .939	& .84$\pm$.01\\
                       %$& \topkavg{2500}  	& \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .991	& .975	& 1.17$\pm$.03\\
                       & \topkavg{2000}  	& \bf 1.00	& \bf 1.00	& \bf 1.00	& .980	& .968	& 1.04$\pm$.02\\
                       %& \topkavg{3000}  	& \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .994	& .981	& 1.31$\pm$.03\\
                       & \topkavg{4000}  	& \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .996	& \bf .987	& 1.64$\pm$.04\\
                       & \topkcomb{5}{200}  	& .979	& .984	& .981	& .892	& .818	& 20.29$\pm$.05\\
                       & \topkcomb{50}{500}   	& \bf .993	& \bf .989	& \bf .994	& .975	& .961	& 21.57$\pm$.06\\
                       %& \topkcomb{50}{1000}   & \bf .993	& \bf .992	& \bf .994	& \bf .987	& .980	& 21.69$\pm$.07\\
                       & \topkcomb{100}{1000}   & \bf 1.00	& \bf .997	& \bf .996	& \bf .993	& \bf .992	& 23.00$\pm$.08\\
                       
  \bottomrule
\end{tabular}
\vspace{0.2em}
\caption{Evaluation of top $K$ retrieval performance, with hit rate (HR) normalized by the brute-force top $K$ method and latency with standard deviation measured over the evaluation of retrieval for a batch of queries (where the batch size is 32). (Relative) hit rate higher than .99 is marked in \textbf{bold}.}
\label{tbl:exp:topk}
\vspace{-1.5em}
\end{center}
\end{table*}

==> table_topk_v3.tex <==
\begin{table*}[ht]
\small 
\vspace{-1em}
\begin{center}
  \begin{tabular}{clllllll}
    \toprule

                        & \bf Method  & \bf HR@1 & \bf HR@5 & \bf HR@10 & \bf HR@50 & \bf HR@100 &  \bf Latency / ms \\                        
    \midrule
    \cut{
\multirow{10}{*}{\mlonem} & \topkbf & 1.00  &	1.00  &	1.00  &	1.00  &	1.00  &	.67$\pm$.03 \\
                       & \topknaive{5}  & .838	& .771	& .683	& .499	& .437	& 1.02$\pm$.05 \\
                       & \topknaive{10}   & .932	& .908	& .844	& .678	& .618	& 1.03$\pm$.05\\
                       & \topknaive{50}   & \bf 1.00	& \bf 1.00	& \bf 1.00	& .978	& .954	& 1.03$\pm$.04\\
                       & \topknaive{100}   & \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .995	& \bf .990	& 1.30$\pm$.03\\
                       & \topkavg{200}   &  .980	& .974	& .970	& .958	& .948	& .82$\pm$.04\\
                       & \topkavg{500}   & \bf .992	& \bf .990	& \bf .991	& \bf .990	& \bf .990	& .80$\pm$.03\\
                       & \topkavg{1000}   &  \bf .996	& \bf .998	& \bf 1.00	& \bf .997	& \bf .999	& .79$\pm$.04\\
                       & \topkcomb{5}{200}  & \bf 1.00	& \bf 1.00	& \bf 1.00	& .997	& .999	& 1.18$\pm$.04 \\
                       %& \topkcomb{50}{500}   & \bf 1.00	& \bf 1.00	& \bf .999	& \bf .999	& \bf .997	& 1.21$\pm$.04  \\
    \midrule

%MoLBruteForceTopK	1.000	1.000	1.000	1.000	1.000	0.67	0.03
%MoLNaiveTopK5	0.838	0.771	0.683	0.499	0.437	1.02	0.05
%MoLNaiveTopK10	0.932	0.908	0.844	0.678	0.618	1.03	0.05
%MoLNaiveTopK50	1.000	1.000	1.000	0.978	0.954	1.03	0.04
%MoLNaiveTopK100	1.000	1.000	1.000	0.995	0.990	1.30	0.03
%MoLAvgTopK200	0.980	0.974	0.970	0.958	0.948	0.82	0.04
%MoLAvgTopK500	0.992	0.990	0.991	0.990	0.990	0.80	0.03
%MoLAvgTopK1000	0.996	0.998	1.000	0.997	0.999	0.79	0.04
%MoLCombTopK5_200	1.000	1.000	1.000	0.997	0.999	1.18	0.04
%MoLCombTopK50_500	1.000	1.000	1.000	0.999	0.999	1.21	0.04
}
\multirow{8}{*}{\mltwentym} & \topkbf & 1.00	& 1.00	& 1.00	& 1.00	& 1.00	& 3.17$\pm$.03\\
                       & \topknaive{5}  & .762	& .707	& .647	& .468	& .402	& 1.28$\pm$.04\\
                       & \topknaive{10}   & .956	& .881	& .820	& .646	& .564	& 1.31$\pm$.04\\
                       & \topknaive{50}   & \bf  1.00	& \bf .992	& .982	& .933	& .900	& 1.63$\pm$.02\\
                       & \topknaive{100}   &	\bf  1.00	& \bf 1.00	& \bf .999	& .981	& .966	& 2.41$\pm$.04 \\
                       & \topkavg{200}   &	\bf  1.00	& \bf .998	& \bf .997	& .982	& .959	& .86$\pm$.04\\
                       & \topkavg{500}   &	\bf  1.00	& \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .998	& .88$\pm$.03\\
                       & \topkcomb{5}{200}    & \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .998	& 1.46$\pm$.04\\
    \midrule

%MoLBruteForceTopK	1.000	1.000	1.000	1.000	1.000	3.17	0.03
%MoLNaiveTopK5	0.762	0.707	0.647	0.468	0.402	1.28	0.04
%MoLNaiveTopK10	0.956	0.881	0.820	0.646	0.564	1.31	0.04
%MoLNaiveTopK50	1.000	0.992	0.982	0.933	0.900	1.63	0.02
%MoLNaiveTopK100	1.000	1.000	0.999	0.981	0.966	2.41	0.04
%MoLAvgTopK200	1.000	0.998	0.997	0.982	0.959	0.86	0.04
%MoLAvgTopK500	1.000	1.000	1.000	0.997	0.993	0.88	0.03
%MoLAvgTopK1000	1.000	1.000	1.000	1.000	0.998	0.86	0.03
%MoLCombTopK5_200	1.000	1.000	1.000	1.000	0.998	1.46	0.04

\multirow{13}{*}{\amzn} & \topkbf & 1.00	& 1.00	& 1.00	& 1.00	& 1.00	& 181.34$\pm$9.09\\
                       & \topknaive{5}  & .907	& .915	& .809	& .509	& .396	& 26.40$\pm$.63\\
%                       & \topknaive{10}    & .936	& \bf .986	& .914	& .698	& .561	& 26.23$\pm$.73\\
                       & \topknaive{50}    & \bf .993	& \bf .992	& \bf .994	& .956	& .902	& 27.59$\pm$.68\\
                       & \topknaive{100}  & \bf 1.00	& \bf .995	& \bf .996	& \bf .985	& .959	& 29.64$\pm$.65\\
                       & \topkavg{200}   	& \bf 1.00	& .978	& .948	& .845	& .767	& 0.81$\pm$.11\\
                       & \topkavg{500}   	& \bf 1.00	& \bf .992	& \bf .996	& .919	& .875	& 0.80$\pm$.09\\
                       & \topkavg{1000}   	& \bf 1.00	& \bf 1.00	& \bf .996	& .963	& .939	& 0.87$\pm$.04\\
                       & \topkavg{2000}  	& \bf 1.00	& \bf 1.00	& \bf 1.00	& .980	& .968	& 1.11$\pm$.04\\
                       & \topkavg{4000}  	& \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .996	& \bf .987	& 1.72$\pm$.04\\
                       & \topkcomb{5}{200}  	& .979	& .984	& .981	& .892	& .818	& 25.73$\pm$.76\\
                       & \topkcomb{50}{500}   	& \bf .993	& \bf .989	& \bf .994	& .975	& .961	& 27.99$\pm$.65\\
                       & \topkcomb{100}{1000}   & \bf 1.00	& \bf .997	& \bf .996	& \bf .993	& \bf .992	& 30.40$\pm$.67\\
    \midrule

%MoLBruteForceTopK	1.000	1.000	1.000	1.000	1.000	181.34	9.09
%MoLNaiveTopK5	0.907	0.915	0.809	0.509	0.396	26.40	0.63
%MoLNaiveTopK10	0.936	0.986	0.914	0.698	0.561	26.23	0.73
%MoLNaiveTopK50	0.993	0.992	0.994	0.956	0.902	27.59	0.68
%MoLNaiveTopK100	1.000	0.995	0.996	0.985	0.959	29.64	0.65
%MoLAvgTopK200	1.000	0.978	0.948	0.845	0.767	0.81	0.11
%MoLAvgTopK500	1.000	0.992	0.996	0.919	0.875	0.80	0.09
%MoLAvgTopK1000	1.000	1.000	0.996	0.963	0.939	0.87	0.04
%MoLAvgTopK2000	1.000	1.000	1.000	0.980	0.968	1.11	0.04
%MoLAvgTopK4000	1.000	1.000	1.000	0.996	0.987	1.72	0.04
%MoLCombTopK5_200	1.000	1.000	1.000	0.996	0.987	25.73	0.76
%MoLCombTopK50_500	0.993	0.989	0.994	0.975	0.961	27.99	0.65
%MoLCombTopK100_1000	1.000	0.997	0.996	0.993	0.992	30.40	0.67

                       
\multirow{7}{*}{\nq} & \topkbf & 1.00	& 1.00	& 1.00	& 1.00	& 1.00	& 37.74$\pm$.47\\
                       & \topknaive{5}  & \bf 1.00	& \bf 1.00	& \bf .995	& .961	& \bf 1.00	& 4.71$\pm$.08\\
                       & \topknaive{10}   & \bf 1.00	& \bf 1.00	& \bf 1.00	& .981	& \bf 1.00	& 4.83$\pm$.08\\
                       & \topknaive{50}   & \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf 1.00	& 6.31$\pm$.09\\
                       & \topkavg{100}   &	\bf .999	& \bf .999	& \bf .999	& \bf .998	& \bf .995	& .57$\pm$.05\\
                       & \topkavg{200}   &	\bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .999	& \bf .999	& .66$\pm$.01 \\
                       & \topkcomb{5}{100}    & \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .999	& \bf .999	& 5.28$\pm$.08 \\

%MoLBruteForceTopK	1.000	1.000	1.000	1.000	1.000	37.74	0.47
%MoLNaiveTopK5	1.000	1.000	0.995	0.961	1.000	4.71	0.08
%MoLNaiveTopK10	1.000	1.000	1.000	0.981	1.000	4.83	0.08
%MoLNaiveTopK50	1.000	1.000	1.000	1.000	1.000	6.31	0.09
%MoLAvgTopK100	0.999	0.999	0.999	0.998	0.995	0.57	0.05
%MoLAvgTopK200	1.000	1.000	1.000	0.999	0.999	0.66	0.01
%MoLCombTopK5_100	1.000	1.000	1.000	0.999	0.999	5.28	0.08

  \bottomrule
\end{tabular}
\vspace{0.3em}
\caption{\nlprevision{Evaluation of top $K$ retrieval performance, with hit rate (HR) normalized by the brute-force top $K$ method and latency %with standard deviation (i.e., $\pm$)
measured over %the evaluation of retrieval for
a batch of queries (where the batch size is 32). (Relative) hit rate higher than .99 is marked in \textbf{bold}.}}
\label{tbl:exp:topk}
\vspace{-2em}
\end{center}
\end{table*}

==> table_topk_v4.tex <==
\begin{table*}[ht]
\small 
\vspace{-1em}
\begin{center}
  \begin{tabular}{clllllll}
    \toprule

                        & \bf Method  & \bf HR@1 & \bf HR@5 & \bf HR@10 & \bf HR@50 & \bf HR@100 &  \bf Latency / ms \\                        
    \midrule
    \cut{
\multirow{10}{*}{\mlonem} & \topkbf & 1.00  &	1.00  &	1.00  &	1.00  &	1.00  &	.67$\pm$.03 \\
                       & \topknaive{5}  & .838	& .771	& .683	& .499	& .437	& 1.02$\pm$.05 \\
                       & \topknaive{10}   & .932	& .908	& .844	& .678	& .618	& 1.03$\pm$.05\\
                       & \topknaive{50}   & \bf 1.00	& \bf 1.00	& \bf 1.00	& .978	& .954	& 1.03$\pm$.04\\
                       & \topknaive{100}   & \bf 1.00	& \bf 1.00	& \bf 1.00	& \bf .995	& \bf .990	& 1.30$\pm$.03\\
                       & \topkavg{200}   &  .980	& .974	& .970	& .958	& .948	& .82$\pm$.04\\
                       & \topkavg{500}   & \bf .992	& \bf .990	& \bf .991	& \bf .990	& \bf .990	& .80$\pm$.03\\
                       & \topkavg{1000}   &  \bf .996	& \bf .998	& \bf 1.00	& \bf .997	& \bf .999	& .79$\pm$.04\\
                       & \topkcomb{5}{200}  & \bf 1.00	& \bf 1.00	& \bf 1.00	& .997	& .999	& 1.18$\pm$.04 \\
                       %& \topkcomb{50}{500}   & \bf 1.00	& \bf 1.00	& \bf .999	& \bf .999	& \bf .997	& 1.21$\pm$.04  \\
    \midrule

%MoLBruteForceTopK	1.000	1.000	1.000	1.000	1.000	0.67	0.03
%MoLNaiveTopK5	0.838	0.771	0.683	0.499	0.437	1.02	0.05
%MoLNaiveTopK10	0.932	0.908	0.844	0.678	0.618	1.03	0.05
%MoLNaiveTopK50	1.000	1.000	1.000	0.978	0.954	1.03	0.04
%MoLNaiveTopK100	1.000	1.000	1.000	0.995	0.990	1.30	0.03
%MoLAvgTopK200	0.980	0.974	0.970	0.958	0.948	0.82	0.04
%MoLAvgTopK500	0.992	0.990	0.991	0.990	0.990	0.80	0.03
%MoLAvgTopK1000	0.996	0.998	1.000	0.997	0.999	0.79	0.04
%MoLCombTopK5_200	1.000	1.000	1.000	0.997	0.999	1.18	0.04
%MoLCombTopK50_500	1.000	1.000	1.000	0.999	0.999	1.21	0.04
}
\multirow{8}{*}{\mltwentym} & \topkbf & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 2.73$\pm$0.01 \\

                       & \topknaive{5}  & 0.691          & 0.670          & 0.626          & 0.462          & 0.399          & 1.61$\pm$0.05 \\

                       & \topknaive{10}   & 0.947          & 0.877          & 0.822          & 0.647          & 0.568          & 1.65$\pm$0.06 \\

                       & \topknaive{50}   & \textbf{1.000} & \textbf{1.000} & \textbf{0.993} & 0.947          & 0.916          & 1.64$\pm$0.05 \\

                       & \topknaive{100}   &	\textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{0.988} & 0.975          & 2.31$\pm$0.02 \\

                       & \topkavg{200}   &	\textbf{0.998} & \textbf{0.997} & \textbf{0.998} & \textbf{0.986} & 0.965          & 1.19$\pm$0.04 \\

                       & \topkavg{500}   &  \textbf{0.998} & \textbf{0.999} & \textbf{0.999} & \textbf{0.999} & \textbf{0.996} & 1.22$\pm$0.05 \\
                       & \topkcomb{5}{200}    & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{0.999} & \textbf{0.996} & 1.86$\pm$0.06 \\
    \midrule

\multirow{16}{*}{\amzn} & \topkbf & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 128.36$\pm$0.30 \\
                       & \topknaive{5}  & \textbf{1.000} & 0.922          & 0.903          & 0.606          & 0.475          & 20.47$\pm$0.07 \\
                       & \topknaive{50}    & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.984          & 0.929          & 21.60$\pm$0.08 \\
                       & \topknaive{100}  & \textbf{1.000} & \textbf{0.997} & \textbf{1.000} & \textbf{0.988} & 0.965          & 23.32$\pm$0.08 \\
                       & \topknaive{200}  & \textbf{1.000} & \textbf{0.997} & \textbf{1.000} & \textbf{0.998} & \textbf{0.995} & 26.55$\pm$0.12 \\
                       & \topkavg{200}   	& 0.966 & 0.916 & 0.905 & 0.761 & 0.666          & 1.13$\pm$0.04 \\
                       & \topkavg{500}   	& 0.966 & 0.977 & 0.965 & 0.858 & 0.813 & 1.17$\pm$0.04 \\
                       & \topkavg{1000}   	& \textbf{0.986} & 0.984 & \textbf{0.995} & 0.918 & 0.877 & 1.12$\pm$0.05 \\
                       & \topkavg{2000}  	& \textbf{1.000} & \textbf{0.992} & \textbf{0.996} & 0.948          & 0.921          & 1.20$\pm$0.02 \\
                       & \topkavg{4000}  	& \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.956          & 0.948          & 2.05$\pm$0.01 \\
                       & \topkavg{8000}       & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.974          & 0.966          & 3.79$\pm$0.01 \\
                       & \topkcomb{5}{200}  	& \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.956          & 0.948          & 20.75$\pm$0.07 \\
                       & \topkcomb{50}{500}   	& \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{0.992} & 0.955          & 22.12$\pm$0.07 \\
                       & \topkcomb{100}{1000}   & \textbf{1.000} & \textbf{0.997} & \textbf{1.000} & \textbf{0.991} & 0.983          & 24.02$\pm$0.13 \\
                       & \topkcomb{200}{2000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{0.996} & 28.01$\pm$0.11 \\
    \midrule

\multirow{7}{*}{\nq} & \topkbf & 1.000	& 1.000	& 1.000	& 1.000	& 1.000	& 37.74$\pm$.47\\
                       & \topknaive{5}  & \bf 1.000	& \bf 1.000	& \bf 0.995	& 0.961	& \bf 1.000	& 4.71$\pm$0.08\\
                       & \topknaive{10}   & \bf 1.000	& \bf 1.000	& \bf 1.000	& 0.981	& \bf 1.000	& 4.83$\pm$0.08\\
                       & \topknaive{50}   & \bf 1.000	& \bf 1.000	& \bf 1.000	& \bf 1.000	& \bf 1.000	& 6.31$\pm$0.09\\
                       & \topkavg{100}   &	\bf 0.999	& \bf 0.999	& \bf 0.999	& \bf 0.998	& \bf 0.995	& 0.57$\pm$0.05\\
                       & \topkavg{200}   &	\bf 1.000	& \bf 1.000	& \bf 1.000	& \bf 0.999	& \bf 0.999	& 0.66$\pm$0.01 \\
                       & \topkcomb{5}{100}    & \bf 1.000	& \bf 1.000	& \bf 1.000	& \bf 0.999	& \bf 0.999	& 5.28$\pm$0.08 \\

%MoLBruteForceTopK	1.000	1.000	1.000	1.000	1.000	37.74	0.47
%MoLNaiveTopK5	1.000	1.000	0.995	0.961	1.000	4.71	0.08
%MoLNaiveTopK10	1.000	1.000	1.000	0.981	1.000	4.83	0.08
%MoLNaiveTopK50	1.000	1.000	1.000	1.000	1.000	6.31	0.09
%MoLAvgTopK100	0.999	0.999	0.999	0.998	0.995	0.57	0.05
%MoLAvgTopK200	1.000	1.000	1.000	0.999	0.999	0.66	0.01
%MoLCombTopK5_100	1.000	1.000	1.000	0.999	0.999	5.28	0.08

  \bottomrule
\end{tabular}
\vspace{0.3em}
\caption{\nlprevision{Evaluation of top $K$ retrieval performance, with hit rate (HR) normalized by the brute-force top $K$ method and latency %with standard deviation (i.e., $\pm$)
measured over %the evaluation of retrieval for
a batch of queries (where the batch size is 32). (Relative) hit rate higher than .99 is marked in \textbf{bold}.}}
\label{tbl:exp:topk}
\vspace{-2em}
\end{center}
\end{table*}
